APE-then-QE: Correcting then Filtering Pseudo Parallel Corpora for MT Training Data Creation

Automatic Post-Editing (APE) is the task of automatically identifying and correcting errors in the Machine Translation (MT) outputs. We propose a repair-filter-use methodology that uses an APE system to correct errors on the target side of the MT training data. We select the sentence pairs from the original and corrected sentence pairs based on the quality scores computed using a Quality Estimation (QE) model. To the best of our knowledge, this is a novel adaptation of APE and QE to extract quality parallel corpus from the pseudo-parallel corpus. By training with this filtered corpus, we observe an improvement in the Machine Translation system's performance by 5.64 and 9.91 BLEU points, for English-Marathi and Marathi-English, over the baseline model. The baseline model is the one that is trained on the whole pseudo-parallel corpus. Our work is not limited by the characteristics of English or Marathi languages; and is language pair-agnostic, given the necessary QE and APE data.

==> 0-abstract.tex <==
\begin{abstract}
Automatic Post-Editing (APE) is the task of automatically identifying and correcting errors in the Machine Translation (MT) outputs. We propose a \textit{repair-filter-use} methodology that uses an APE system to correct errors on the target side of the MT training data. We select the sentence pairs from the original and corrected sentence pairs based on the quality scores computed using a Quality Estimation (QE) model. To the best of our knowledge, this is a novel adaptation of APE and QE to extract quality parallel corpus from the pseudo-parallel corpus. By training with this filtered corpus, we observe an improvement in the Machine Translation system's performance by \textbf{5.64} and \textbf{9.91} BLEU points, for English-Marathi and Marathi-English, over the baseline model. The baseline model is the one that is trained on the whole pseudo-parallel corpus. \textit{Our work is not limited by the characteristics of English or Marathi languages; and is language pair-agnostic, given the necessary QE and APE data.}

\end{abstract}


==> 1-introduction.tex <==
\section{Introduction}
The performance of machine translation systems has experienced significant advancements with the introduction of Neural Machine Translation (NMT) models. However, these NMT models are data-hungry. In order to train high-quality NMT systems, we require a parallel corpus that is not only abundant but also of excellent quality \cite{akshay}. But NMT for low-resource languages is difficult due to the unavailability of  high-quality parallel data. Hence, we have to rely on the noisy web-crawled corpora for low-resource languages. The task of \textbf{Parallel Corpus Filtering} aims to provide a scoring mechanism that helps extract good-quality parallel corpus from a noisy pseudo-parallel corpus. The task of \textbf{Automatic Post Editing} (APE) task aims to automatically identify and correct errors in MT outputs. The task of \textbf{Quality Estimation} (QE) aims to provide a quality score for a translation when the reference translation is unavailable. Our \textbf{motivation} is as follows: As the APE with QE systems has yet to be investigated for error correction in noisy pseudo-parallel corpora, this encourages us to utilize them to enhance the quality of the pseudo-parallel corpus. We use the APE model to rectify errors in the target side of the noisy pseudo-parallel corpus. Next, we employ Quality Estimation to assign quality scores to the sentence pairs present in the original and corrected pseudo-parallel corpus and select the parallel sentences with the highest quality scores. We aim to improve the quality of Machine Translation for the English (En) - Marathi (Mr) language pair by  using an APE model to rectify errors on the target side of the pseudo-parallel corpus. We observe that APE and QE-assisted corpus filtering significantly improves the performance of the En-Mr MT system. We restrict our experiments solely to the En-Mr language pair due to a lack of APE and QE resources.\\
\indent Our contributions are:
\begin{enumerate}
    \item \textbf{Adaption of APE-then-QE},  we initially calculate QE scores for the original pseudo-parallel corpus. Next, we apply Automatic Post-Editing (APE) to the target side of the pseudo-parallel corpus and calculate QE scores for the resulting APE-edited pseudo-parallel corpus. Based on these scores, we determine whether to utilize the APE-edited sentence pairs or stick with the original sentence pairs when training the Neural Machine Translation (NMT) systems, shown in figure \ref{img:ape qe dia}. To the best of our knowledge, this is a novel adaptation of APE and QE for extracting quality parallel corpus from the pseudo-parallel corpus. 
    
    % \item \textbf{Adaptation of APE-then-QE} (i) to correct errors on the target side of the pseudo-parallel corpus using Automatic Post-Editing and (ii) to select the best sentence pairs from the corrected and original pseudo-parallel corpus using Quality Estimation shown in figure \ref{img:ape qe dia};  to the best of our knowledge, this is a novel adaptation of APE and QE for extracting quality parallel corpus from the pseudo-parallel corpus.
    
    \item Demonstration of \textbf{performance improvement} of the Machine Translation systems by \textbf{5.64} and \textbf{9.91} BLEU points for English-Marathi and Marathi-English language pairs, over the model trained on the whole pseudo-parallel corpus, shown in table \ref{tab:4}; the choice of language pairs was dictated by the availability of APE and QE data, manually created for English-Marathi pairs.
    
\end{enumerate}

==> 2-related-work.tex <==
\section{Related Work}
\subsection{Parallel Corpus Filtering}
Neural Machine Translation (NMT) is extremely \textit{data hungry}~\cite{sutskever2014sequence, bahadanau, NIPS2017_3f5ee243}. \citet{herold-etal-2022-detecting} studied various types of noise
present in the Pseudo-Parallel corpora and investigated if the current filtering systems remove all
types of noise.
% The Conference on Machine Translation (WMT) has organized annual Shared Tasks on Parallel Corpus Filtering (WMT 2018, WMT 2019, WMT 2020).\\
% ~\citet{labse} proposed the LaBSE model, which is a multilingual sentence embedding model trained on 109 languages, including some Indic languages.\\
\indent Recently,~\citet{akshay} used a Phrase Pair Injection with LaBSE~\cite{labse} based Corpus Filtering to extract high-quality parallel data from a noisy parallel corpus.~\citet{briakou-etal-2022-bitextedit} proposed an approach to reconstruct the original translations and translate, in a multi-task fashion, and use it to automatically edit the mined corpus. They train a multi-task model using synthetic supervision from mined bitexts. They show improvement in the bitext quality of the CCMatrix corpus. In contrast, we use a different training strategy to train the APE systems, namely, Curriculum Training Strategy \cite{deoghare-bhattacharyya-2022-iit}. \citet{batheja2023a} proposed a Quality Estimation based corpus filtering approach that performed better than all previously proposed methods. In contrast, we use APE and QE-assisted filtering to correct and extract high-quality data from noisy pseudo-parallel data.  

% \subsection{Quality Estimation}
% Quality Estimation (QE) is the task of evaluating the quality of a translation when reference translation is not available. The state-of-the-art MonoTransQuest architecture, proposed by~\citet{ranasinghe-etal-2020-transquest}, builds upon XLM-R, a widely-used pre-trained cross-lingual language model known for its ability to generalize to low-resource languages~\cite{conneau-etal-2020-unsupervised}.~\citet{kocyigit-etal-2022-better} proposed a combination of multitask training, data augmentation
% and contrastive learning to achieve better and
% more robust QE, in Parallel Corpus Mining setting. 
% The Parallel Corpus Mining task aims to detect
% the most similar texts in a large multilingual collection and perform sentence alignment. This motivates us to use QE in the Parallel Corpus Filtering task.

\subsection{Automatic Post Editing}
Automatic Post-Editing (APE) is an auxiliary task in a Machine Translation (MT) field, which is aimed at automatically identifying and correcting MT output errors~\cite{chatterjee-etal-2020-findings}. APE systems have the potential to reduce human effort by correcting systematic and repetitive translation errors~\cite{laubli-etal-2013-assessing, pal-etal-2016-multi}. Recent APE approaches utilize transfer learning by adapting pre-trained language or translation models to perform APE~\cite{lopes-etal-2019-unbabels, wei-etal-2020-hw, sharma-etal-2021-adapting}. Also, the recent approaches use multilingual or cross-lingual models to get latent representations of the source and target sentences~\cite{lee-etal-2020-postech}.~\citet{oh-etal-2021-netmarble} have shown that gradually adapting pre-trained models to APE by using the Curriculum Training Strategy (CTS) improves performance.~\citet{deoghare-bhattacharyya-2022-iit} showed that augmenting the APE data with phrase-level APE triplets improves feature diversity, and using a QE system allows for identification and discarding poor-quality APE outputs.  We use the APE system to rectify errors in the target side of the noisy pseudo-parallel corpus.



% Unlike the current work, the authors compared sentence-level QE predictions for the original translation and the corresponding APE-generated version, to decide whether the APE-generated version is an improved version of the original translation or not.

\begin{figure*}
\begin{center}
\includegraphics[width=\textwidth]{Images/EMNLP23.png}
\caption{The proposed APE-then-QE based corpus filtering pipeline.}
\label{img:ape qe dia}
\end{center}
\end{figure*}

==> 3-approaches.tex <==
% \begin{table*}[t]
%     \centering
%     \begin{tabular}{ |p{4cm}||p{2cm}|p{3cm}|p{3cm}|  }
%      \hline
%     %  \multicolumn{4}{|c|}{Country List} \\
%     %  \hline
%       \multicolumn{2}{|c|}{\textbf{Corpus Name}}& \textbf{Train}(\# of Sentence Pairs)& \textbf{Validation}(\# of Sentence Pairs)\\
%      \hline
%      \multirow{4}{*}{\textbf{Combined Corpus}}&\textbf{ILCI}& 46,277 & \multirow{4}{*}{3,999} \\
%      &  \textbf{PMI}&28,973&\\
%      & \textbf{PIB}&1,08,219&\\
%      & \textbf{Bible}&58,375 &\\
%      & \textbf{Tatoeba}&3,66,144&\\
%      \hline
%      \multicolumn{2}{|c|}{\textbf{Samanantar}}& 1,985,481&-\\
%      \hline
%      \multicolumn{2}{|c|}{\textbf{Total Corpus size}}& 2,593,469&3,999\\
%     \hline
%     \end{tabular}
%     \caption{Hindi-Marathi Corpora Statistics}
%     \label{lab:corpus}
% \end{table*}
% \begin{figure}[t]
% \begin{center}
% \includegraphics[scale=.4]{Images/emnlp_last.png}\caption{Phrase Pair Injection with LaBSE Filtering Pipeline}
% \label{fig:1}
% \end{center}
% \end{figure}

\section{Approaches}
% \subsection{LaBSE based Filtering \cite{akshay}}
% \cite{labse} proposed a Language Agnostic BERT Sentence Embedding model that supports 109 languages, including some Indic languages. We use  LaBSE\footnote{\url{https://huggingface.co/sentence-transformers/LaBSE}} to generate the source and target sentence embeddings for the pseudo-parallel corpora. Then, we extract high quality parallel sentences from pseudo-parallel corpora based on the cosine similarity computed between the source and target sentence embeddings.
\subsection{Phrase Pair Injection (PPI) with LaBSE-based Filtering \cite{akshay}}
~\citet{akshay} proposed a combination of Phrase Pair Injection~\cite{sen2021neural} and LaBSE-based Corpus Filtering to extract high-quality parallel data from a pseudo-parallel corpus. We train a PBSMT model on the pseudo-parallel corpus using the \textit{Moses} \footnote{\url{http://www2.statmt.org/moses/?n=Development.GetStarted}} decoder. Then, we extract the longest unique phrase pairs with the highest translation probability. We use  LaBSE\footnote{\url{https://huggingface.co/sentence-transformers/LaBSE}} to generate the source and target sentence embeddings for the pseudo-parallel corpora. Then, we extract high-quality parallel sentences from pseudo-parallel corpora based on the cosine similarity computed between the source and target sentence embeddings. We apply the same process on the longest unique phrase pairs and extract LaBSE-filtered high-quality phrase pairs. We augment these high-quality phrase pairs with LaBSE-filtered parallel sentences. 
\subsection{Quality Estimation (QE) based Filtering \cite{batheja2023a}}
\citet{batheja2023a} proposed Quality Estimation based Filtering approach to extract high-quality parallel corpus from noisy pseudo-parallel corpus using threshold QE score values. We borrow their En-Mr sentence level QE model to perform QE based Filtering.
\subsection{Our Approach, APE-then-QE based Filtering}
\citet{deoghare-bhattacharyya-2022-iit} proposed a curriculum training strategy to train the APE system. We borrow the same training strategy to train our En-Mr APE system. The training details are mentioned in \ref{app:training details}.\\
\indent We use the trained APE system to correct errors in the target side of the noisy pseudo-parallel corpus. As APE systems are prone to the problem of ‘over-correction’, we use a sentence-level quality estimation (QE) system to select the final output between an original target sentence and the corresponding output generated by the APE model. We compare our approach against three previously proposed approaches, namely, \textbf{LaBSE based Filtering, LaBSE + PPI with LABSE based Filtering and QE based Filtering.}

==> 4-experiments.tex <==
\section{Experimental Setup} \label{experiment setup}
\begin{table}[htp]
\centering
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{llr}
\hline
\textbf{Corpus Name} & \textbf{\# Samples} &\textbf{Type}\\
\hline
% \multirow{3}{*}{\textbf{Parallel Corpus}} &Hindi-Bengali& 3.6M \\
\textbf{APE data}&18K triplets& Real\\ \hline

 \textbf{Parallel Corpus}&6M pairs&\multirow{3}{*}{Synthetic}\\ 
 \textbf{Phrase-Level Data} & 60K triplets&\\
 \textbf{APE data}& 2.5M triplets\\ \hline
 % &Chinese-English&24.7M\\\hline
% Total & 25.9L \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Dataset Statistics for the task of Automatic Post Editing for En-Mr language pair}
\label{tab:apedata}
\end{table}

\begin{table*}[htp]
% \small
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrr}
\hline
\textbf{Technique} & \textbf{\# Sentence Pairs (in Millions)}& \textbf{En$\rightarrow$Mr} & \textbf{Mr$\rightarrow$En}\\ \hline
\textbf{APE-then-QE based Filtering} & 3.5M & \textbf{14.44} & \textbf{25.81}\\
\textbf{APE based Filtering} & 3.5M &14.28&  24.43\\
 \textbf{QE based Filtering}& 2.61M &9.4 & 17.7\\
 \cite{batheja2023a}&&&\\
 \textbf{PPI with LaBSE  based Filtering} & 4.09M& 9.9 & 17.0 \\
 \cite{akshay}&&&\\
 \textbf{LaBSE based Filtering} & 2.85M &  8.8 & 16.7\\
 \cite{akshay}&&&\\
 \textbf{Baseline}& 3.5M& 8.8 & 15.9\\ \hline
 % \textbf{Baseline} &  5.1 & 10.2 & 12.4 & 19.66 & 2.85   
\end{tabular}
}
\caption{BLEU scores of NMT models on FLORES101 test data. For actual instances of translations please refer to Appendix \ref{instances}}
\label{tab:4}
\end{table*}

\subsection{Dataset}\label{dataset}
In all NMT experiments, we use two sets of corpus, namely, Parallel and Pseudo-Parallel corpus. The En-Mr \textbf{Parallel corpus} consists of 248K high-quality sentence pairs, which include the ILCI phase 1, Bible, PIB, and PM-India corpus~\cite{ilci, bible, pmi}. The En-Mr \textbf{Pseudo-Parallel} corpus contains 3.28M sentence pairs of varying quality from the Samanantar Corpus~\cite{samanantar}. \\
% \indent In QE experiments, we use the QE data used by~\citet{deoghare-bhattacharyya:2022:WMT} for the En-Mr language pair. The En-Mr QE data consists of human-annotated z-standardized Direct Assessment (DA) scores. The train, dev and test instances of QE data are 26K, 1K and 1K, respectively.\\
\indent We use the WMT22 En-Mr APE shared task data to develop the APE system~\cite{bhattacharyya-etal-2022-findings}. The statistics are listed in Table~\ref{tab:apedata}. The train set consists of 18K APE triples \textit{<source, MT  output, reference>} generated with the help of professional post-editors. We also use synthetically generated 2.5M APE triplets. The NMT model, which we train as a step in the CTS, is trained using the publically available parallel corpora (Samanantar~\cite{samanantar}, Anuvaad, Tatoeba, and ILCI~\cite{bansal2013corpora}) containing around 6M sentence pairs. The detailed APE data statistics are mentioned in table \ref{tab:apedata}. The annotation guidelines for the task of APE are mentioned in the \textbf{Appendix} \ref{annotation}.

\indent For evaluation, we use the FLORES 101 test set, which contains 1,012 sentence pairs for the En-Mr language pair.
% \subsection{Baseline}
% We train the baseline models for English-Marathi, Hindi-Bengali, Chinese-English directly on their respective parallel corpus.

\subsection{Models}
\label{models}
We use a Transformer based architecture to train the NMT models for all our experiments. We use MonoTransQuest model architecture to train the QE models. The training details and model architecture is mentioned in \textbf{Appendix} \ref{app:model arch} and \ref{app:training details}.\\
% \begin{itemize} respectively.
\noindent \textbf{Baseline:} We train the baseline NMT models on the whole pseudo-parallel corpus augmented with the parallel corpus for the En-Mr language pair.\\
\noindent \textbf{LaBSE based Filtering:} In this model, we use the LaBSE filtering with threshold \textbf{0.8} to extract good quality parallel sentences from the En-Mr pseudo-parallel corpus. Then, we augment the parallel corpus with the LaBSE-filtered parallel sentences and train the respective NMT models. \\
\noindent \textbf{PPI with LaBSE based Filtering:} We perform Phrase Pair Injection with LaBSE-based Filtering to train the respective NMT models. This involves extracting LaBSE-filtered parallel sentences and phrases from the pseudo-parallel corpus and augmenting them with the parallel corpora. We train this model for the purpose of comparing it with our proposed best model.\\
\noindent \textbf{QE based Filtering:} We use the En-Mr sentence level QE model provided by \cite{batheja2023a} to compute the quality scores for the pseudo-parallel corpora. Then, we extract high-quality sentence pairs from the pseudo-parallel corpus using the threshold value of \textbf{-0.5} for the En-Mr language pair. We augment the extracted high-quality sentence pairs with the parallel corpus and train the respective NMT models.\\
\noindent \textbf{Our Model, APE based Filtering:} We train an APE system for the En-Mr language pair and use it to correct errors in the target side of a noisy pseudo-parallel corpus. We augment the corrected pseudo-parallel corpus with the parallel corpus and use it to train the NMT models. \\  
\noindent \textbf{Our Model, APE-then-QE based Filtering:} First, we train an APE system for the En-Mr language pair. This APE system is then used to correct errors in the target side of a noisy pseudo-parallel corpus. Next, we use a sentence-level QE system to choose the final target sentence, either the original or the corresponding output generated by the APE model. Finally, we augment the corrected pseudo-parallel corpus with the parallel corpus and use it to train the NMT models.

==> 5-evaluation.tex <==
\section{Results and Analysis}
We evaluate our NMT models using BLEU~\cite{papineni-etal-2002-bleu}. We use sacrebleu~\cite{sacrebleu} python library to calculate the BLEU scores. Table \ref{tab:4} shows that \textbf{APE-then-QE based filtering} model outperforms all other models for the En-Mr language pair. The \textbf{APE-then-QE based filtering} model improves the MT system's performance by \textbf{5.64} and \textbf{9.91} BLEU points over the \textbf{baseline} model for En$\rightarrow$Mr and Mr$\rightarrow$En, respectively. It also outperforms \textbf{QE based Filtering} and \textbf{LaBSE + PPI-LaBSE based Filtering} model by \textbf{5.04}, \textbf{8.11} BLEU points for En$\rightarrow$Mr and \textbf{4.54}, \textbf{8.81} BLEU points for Mr$\rightarrow$En, respectively.\\
\indent We observe a significant improvement in the En-Mr NMT system by \textbf{5.48} and \textbf{8.53} BLEU points over the baseline, merely by correcting errors in the target side of the noisy pseudo-parallel corpus using the En-Mr APE system. Furthermore, we have also discovered that utilizing QE-based sentence selection alongside APE-based pre-editing of the pseudo-parallel corpus resulted in a further enhancement of the En-Mr NMT system by \textbf{0.16} and \textbf{1.38} BLEU points when compared to the \textbf{APE-based filtering model}. 


==> 6-Conclusion.tex <==
\section{Conclusion and Future Work}
In this work, we show that correcting errors in the target side of the noisy pseudo-parallel corpus using an APE model and selecting high-quality sentence pairs from the original and corrected sentence pairs using QE helps NMT models improve their performance significantly.
Also, the proposed approach is independent of the properties of English and Marathi languages and can be applied to any language pair. However, our language pair-agnostic approach requires APE and QE data to correct and filter noise from pseudo-parallel data. \\
% Also, the proposed approach is independent of language-specific properties. It can be applied to any language pair if the necessary QE and APE data is available. \\
\indent In the future, we will use the proposed approach and analyze data from other language pairs. We also plan to use a combination of word and sentence level QE to select high-quality sentence pairs between original and APE-corrected sentence pairs.

% \section{Acknowledgements}
% We would like to thank the anonymous reviewers for their insightful feedback. We also express our gratitude towards Shivam Mhaskar, Sourabh Deoghare, Jyotsana Khatri, and other members of the Machine Translation group at CFILT, IIT Bombay, for their interesting and insightful comments.
\section*{Limitations}
Developing APE and QE systems involves using human-annotated data, which can be costly and time-consuming. We restrict our experiments solely to the En-Mr language pair due to a lack of APE and QE resources. The QE-based filtering experiments involve a hyper-parameter called ``threshold quality score''. One of our limitations is the usual one, namely finding the correct set of hyperparameters through a large number of experiments.
\section*{Ethics Statement}
The aim of our work is to improve the quality of En-Mr MT systems by using APE and QE models to rectify errors on the target side of the pseudo-parallel corpus and extract high-quality parallel corpus. The datasets that we used in this work are publicly available, and we have cited the sources of all the datasets that we have used.  Publicly available datasets can contain biased sentences.

% In this work, we have implemented and compared various parallel corpus filtering techniques to improve the task of Machine Translation for the language pair Hindi-Marathi. We have shown that the combination of statistical and neural parallel corpus filtering makes the best utilization of the noisy corpus. This technique helped us to significantly improve the quality of Hindi-Marathi translations over the baseline.\\
% \indent In future, we plan to use these filtering techniques for other language pairs. This will provide us a general overview of how these filtering techniques perform on multiple languages. We also plan to explore other filtering techniques which uses GPT-2 and GPT-3 language models. We anticipate improvements in the result by trying different threshold values in the LaBSE filtering.
